Wasserstein Robust Classification with Fairness Constraints

We propose a distributionally robust classification model with a fairness constraint that encourages the classifier to be fair in view of the equality of opportunity criterion. We use a type-$\infty$ Wasserstein ambiguity set centered at the empirical distribution to model distributional uncertainty and derive a conservative reformulation for the worst-case equal opportunity unfairness measure. We establish that the model is equivalent to a mixed binary optimization problem, which can be solved by standard off-the-shelf solvers. To improve scalability, we further propose a convex, hinge-loss-based model for large problem instances whose reformulation does not incur any binary variables. Moreover, we also consider the distributionally robust learning problem with a generic ground transportation cost to hedge against the uncertainties in the label and sensitive attribute. Finally, we numerically demonstrate that our proposed approaches improve fairness with negligible loss of predictive accuracy.

==> Wasserstein Robust Classification with Fairness Constraints/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> Wasserstein Robust Classification with Fairness Constraints/style.tex <==
%================================ Packages =====================================
%\usepackage[round]{natbib}
\usepackage[colorlinks=true, linkcolor=red,citecolor=blue]{hyperref}
\usepackage{multirow}
\usepackage{tcolorbox}
\usepackage{wrapfig}
\usepackage{amssymb, amsthm, amsmath, amsfonts}
\usepackage{mathtools, longfbox, dsfont, mathrsfs, color, bm, enumitem, url, upgreek}
\usepackage{graphicx, transparent, wrapfig}
\usepackage{caption}
\usepackage{subcaption}
% \usepackage{subfig}
%\usepackage[ruled,vlined]{algorithm2e}
% \usepackage{titlesec}
\usepackage{multicol}
\usepackage{algorithm, algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\usepackage{tcolorbox}
\usepackage{bbm}


% \titlelabel{\thetitle.\;}
%===============================================================================

%============================== Abbreviation ===================================
\DeclareMathOperator{\Tr}{tr}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\viet}[1]{\begin{tcolorbox}[width=\textwidth, colframe=blue
, boxrule=0.5pt, boxsep=0.001mm]{{\footnotesize{Viet: #1}}}\end{tcolorbox}}
\newcommand{\yijie}[1]{\begin{tcolorbox}[width=\textwidth, colframe=red
, boxrule=0.5pt, boxsep=0.001mm]{{\footnotesize{Yijie: #1}}}\end{tcolorbox}}
\newcommand{\grani}[1]{\begin{tcolorbox}[width=\textwidth, colframe=yellow
, boxrule=0.5pt, boxsep=0.001mm]{{\footnotesize{Grani: #1}}}\end{tcolorbox}}

\newcommand{\Let}{\triangleq}
\newcommand{\Pnom}{\hat \PP} 
\newcommand{\supp}{\textrm{supp}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}
\newcommand{\mbb}{\mathbb}
\newcommand{\Wass}{\mathds W}
\newcommand{\VV}{\mathds V}
\newcommand{\opt}{^\star}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle }
\newcommand{\ds}{\displaystyle}

\newcommand{\defeq}{\coloneqq}
\newcommand{\pd}{\mathbbm{P}}
\newcommand{\ie}{\textit{i.e., }}
\newcommand{\R}{\mathbb{R}}
\newcommand{\wh}{\hat}
\newcommand{\dist}{\textrm{\textbf{dist}}}
\newcommand{\mc}{\mathcal}
\newcommand{\m}{\mathcal{M}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\x}{\mathcal{X}}
\newcommand{\y}{\mathcal{Y}}
\newcommand{\asinh}{\textrm{arcsinh}}
\newcommand{\samplerate}{\mathcal{O}}
\newcommand{\cdf}{F}
\newcommand{\bs}{\boldsymbol}
\newcommand{\ctransj}{\dvy_j-c(x,y_j)}
\newcommand{\ctransjneg}{-\dvy_j+c(x,y_j)}
\newcommand{\euler}{\gamma}
\newcommand{\DS}{\displaystyle}
\newcommand{\st}{\mathrm{s.t.}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eps}{\varepsilon}
%===============================================================================

%================================ Theorem ======================================
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%===============================================================================

%============================== Figures Path ===================================
\graphicspath{{figures/}}
%===============================================================================

%============================== Modify style ===================================
\usepackage[utf8]{inputenc}    % allow utf-8 input
\usepackage[T1]{fontenc}       % use 8-bit T1 fonts
\usepackage{tabularx}
\usepackage{lmodern}           % allow pdf compability
\usepackage{xcolor}
% \hypersetup{
% 	colorlinks,
% 	linkcolor={blue!55!black},
% 	citecolor={red!55!black},
% 	urlcolor={blue!80!black}
% }

% ================== Margins & Layout =================================
% \addtolength{\voffset}{0cm} 
% \addtolength{\textheight}{1cm} 
% \addtolength{\hoffset}{-2cm}
% \addtolength{\textwidth}{4cm}

% \setlength{\parskip}{1mm}
% \linespread{1.12}
\usepackage[margin=1in]{geometry}
%===============================================================================
\graphicspath{{graph/}}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
